Linear-Quadratic Optimal Control in Maximal Coordinates

The linear-quadratic regulator (LQR) is an efficient control method for linear and linearized systems. Typically, LQR is implemented in minimal coordinates (also called generalized or "joint" coordinates). However, other coordinates are possible and recent research suggests that there may be numerical and control-theoretic advantages when using higher-dimensional non-minimal state parameterizations for dynamical systems. One such parameterization is maximal coordinates, in which each link in a multi-body system is parameterized by its full six degrees of freedom and joints between links are modeled with algebraic constraints. Such constraints can also represent closed kinematic loops or contact with the environment. This paper investigates the difference between minimal- and maximal-coordinate LQR control laws. A case study of applying LQR to a simple pendulum and simulations comparing the basins of attraction and tracking performance of minimal- and maximal-coordinate LQR controllers suggest that maximal-coordinate LQR achieves greater robustness and improved tracking performance compared to minimal-coordinate LQR when applied to nonlinear systems.

==> plots/pendulumerror.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.85098,0.32549,0.09804}%
\definecolor{mycolor2}{rgb}{0.00000,0.44706,0.74118}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.375in,
height=1.457in,
at={(0.573in,2.417in)},
scale only axis,
xmin=-1.5707963267949,
xmax=1.5707963267949,
xtick={-1.5707963267949,-0.785398163397448,0,0.785398163397448,1.5707963267949},
xticklabels={{-1.57},{-0.79},{0},{0.79},{1.57}},
ymin=0,
ymax=5.62720607985785,
axis background/.style={fill=white},
legend style={at={(0.5,0.97)}, anchor=north, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
-1.64	6.35\\
-1.55	5.41\\
-1.45	4.55\\
-1.35	3.78\\
-1.26	3.1\\
-1.16	2.5\\
-1.06	1.98\\
-0.97	1.53\\
-0.87	1.16\\
-0.77	0.85\\
-0.68	0.61\\
-0.58	0.42\\
-0.48	0.27\\
-0.39	0.17\\
-0.29	0.1\\
-0.19	0.05\\
-0.1	0.02\\
0	0\\
0.1	0.02\\
0.19	0.05\\
0.29	0.1\\
0.39	0.17\\
0.48	0.27\\
0.58	0.42\\
0.68	0.61\\
0.77	0.85\\
0.87	1.16\\
0.97	1.53\\
1.06	1.98\\
1.16	2.5\\
1.26	3.1\\
1.35	3.78\\
1.45	4.55\\
1.55	5.41\\
1.64	6.35\\
};
\addlegendentry{LQR min.}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
-1.64	1.03\\
-1.55	0.95\\
-1.45	0.87\\
-1.35	0.79\\
-1.26	0.72\\
-1.16	0.65\\
-1.06	0.59\\
-0.97	0.52\\
-0.87	0.46\\
-0.77	0.41\\
-0.68	0.35\\
-0.58	0.3\\
-0.48	0.24\\
-0.39	0.19\\
-0.29	0.14\\
-0.19	0.1\\
-0.1	0.05\\
0	0\\
0.1	0.05\\
0.19	0.1\\
0.29	0.14\\
0.39	0.19\\
0.48	0.24\\
0.58	0.3\\
0.68	0.35\\
0.77	0.41\\
0.87	0.46\\
0.97	0.52\\
1.06	0.59\\
1.16	0.65\\
1.26	0.72\\
1.35	0.79\\
1.45	0.87\\
1.55	0.95\\
1.64	1.03\\
};
\addlegendentry{LQR max.}

\end{axis}

\begin{axis}[%
width=3.354in,
height=1.396in,
at={(0.594in,0.615in)},
scale only axis,
xmin=-3.14159265358979,
xmax=0,
xtick={-3.14159265358979,-2.3562,-1.5707963267949,-0.785398163397448,0},
xticklabels={{-3.14},{-2.36},{-1.57},{-0.79},{0}},
ymin=0,
ymax=20,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
-3.19	18.2\\
-3.09	16.99\\
-3	15.79\\
-2.9	14.6\\
-2.8	13.43\\
-2.71	12.28\\
-2.61	11.16\\
-2.51	10.08\\
-2.42	9.05\\
-2.32	8.05\\
-2.22	7.11\\
-2.13	6.22\\
-2.03	5.38\\
-1.93	4.61\\
-1.84	3.9\\
-1.74	3.25\\
-1.64	2.67\\
-1.55	2.15\\
-1.45	1.69\\
-1.35	1.29\\
-1.26	0.96\\
-1.16	0.68\\
-1.06	0.45\\
-0.97	0.27\\
-0.87	0.13\\
-0.77	0.02\\
-0.68	0.05\\
-0.58	0.11\\
-0.48	0.14\\
-0.39	0.17\\
-0.29	0.2\\
-0.19	0.25\\
-0.1	0.31\\
0	0.39\\
};
\addplot [color=mycolor2, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
-3.19	1.26\\
-3.09	1.97\\
-3	2.62\\
-2.9	3.2\\
-2.8	3.69\\
-2.71	4.11\\
-2.61	4.45\\
-2.51	4.71\\
-2.42	4.9\\
-2.32	5.02\\
-2.22	5.06\\
-2.13	5.05\\
-2.03	4.97\\
-1.93	4.84\\
-1.84	4.66\\
-1.74	4.43\\
-1.64	4.17\\
-1.55	3.88\\
-1.45	3.56\\
-1.35	3.22\\
-1.26	2.87\\
-1.16	2.51\\
-1.06	2.15\\
-0.97	1.8\\
-0.87	1.46\\
-0.77	1.14\\
-0.68	0.84\\
-0.58	0.56\\
-0.48	0.32\\
-0.39	0.1\\
-0.29	0.07\\
-0.19	0.21\\
-0.1	0.31\\
0	0.36\\
};
\end{axis}

\begin{axis}[%
width=3.088in,
height=3.168in,
at={(0.701in,0.663in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={$\theta$},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={control input error},
axis line style={draw=none},
ticks=none,
title style={font=\bfseries},
title={(c) Error compared to optimal input},
axis x line*=bottom,
axis y line*=left
]
\end{axis}

\begin{axis}[%
width=4.188in,
height=4.188in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\node[below right, align=left]
at (rel axis cs:0.456,0.664) {v = 0};
\node[below right, align=left]
at (rel axis cs:0.456,0.338) {v = 4};
\end{axis}
\end{tikzpicture}%

==> plots/pendulumv0.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.50196,0.50196,0.50196}%
\definecolor{mycolor2}{rgb}{0.85098,0.32549,0.09804}%
\definecolor{mycolor3}{rgb}{0.00000,0.44706,0.74118}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.333in,
height=3.333in,
at={(0.646in,0.594in)},
scale only axis,
xmin=-1.5707963267949,
xmax=1.5707963267949,
xtick={-1.5707963267949,-0.785398163397448,0,0.785398163397448,1.5707963267949},
xticklabels={{-1.57},{-0.79},{0},{0.79},{1.57}},
xlabel style={font=\color{white!15!black}},
xlabel={$\theta$},
ymin=-16,
ymax=16,
ylabel style={font=\color{white!15!black}},
ylabel={$u(\theta)$},
axis background/.style={fill=white},
title style={font=\bfseries},
title={$\text{(a) u(}\theta\text{) for different controllers}$},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, dashed, line width=2.0pt]
  table[row sep=crcr]{%
-1.64	7.34\\
-1.55	7.36\\
-1.45	7.3\\
-1.35	7.18\\
-1.26	7\\
-1.16	6.75\\
-1.06	6.43\\
-0.97	6.06\\
-0.87	5.62\\
-0.77	5.14\\
-0.68	4.61\\
-0.58	4.03\\
-0.48	3.42\\
-0.39	2.77\\
-0.29	2.1\\
-0.19	1.41\\
-0.1	0.71\\
0	0\\
0.1	-0.71\\
0.19	-1.41\\
0.29	-2.1\\
0.39	-2.77\\
0.48	-3.42\\
0.58	-4.03\\
0.68	-4.61\\
0.77	-5.14\\
0.87	-5.62\\
0.97	-6.06\\
1.06	-6.43\\
1.16	-6.75\\
1.26	-7\\
1.35	-7.18\\
1.45	-7.3\\
1.55	-7.36\\
1.64	-7.34\\
};
\addlegendentry{gravity}

\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
-1.64	9.94\\
-1.55	9.92\\
-1.45	9.82\\
-1.35	9.63\\
-1.26	9.35\\
-1.16	9\\
-1.06	8.56\\
-0.97	8.05\\
-0.87	7.46\\
-0.77	6.81\\
-0.68	6.1\\
-0.58	5.33\\
-0.48	4.52\\
-0.39	3.66\\
-0.29	2.78\\
-0.19	1.87\\
-0.1	0.94\\
0	0\\
0.1	-0.94\\
0.19	-1.87\\
0.29	-2.78\\
0.39	-3.66\\
0.48	-4.52\\
0.58	-5.33\\
0.68	-6.1\\
0.77	-6.81\\
0.87	-7.46\\
0.97	-8.05\\
1.06	-8.56\\
1.16	-9\\
1.26	-9.35\\
1.35	-9.63\\
1.45	-9.82\\
1.55	-9.92\\
1.64	-9.94\\
};
\addlegendentry{NL. optimal}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
-1.64	16.29\\
-1.55	15.33\\
-1.45	14.37\\
-1.35	13.41\\
-1.26	12.45\\
-1.16	11.5\\
-1.06	10.54\\
-0.97	9.58\\
-0.87	8.62\\
-0.77	7.66\\
-0.68	6.71\\
-0.58	5.75\\
-0.48	4.79\\
-0.39	3.83\\
-0.29	2.87\\
-0.19	1.92\\
-0.1	0.96\\
0	0\\
0.1	-0.96\\
0.19	-1.92\\
0.29	-2.87\\
0.39	-3.83\\
0.48	-4.79\\
0.58	-5.75\\
0.68	-6.71\\
0.77	-7.66\\
0.87	-8.62\\
0.97	-9.58\\
1.06	-10.54\\
1.16	-11.5\\
1.26	-12.45\\
1.35	-13.41\\
1.45	-14.37\\
1.55	-15.33\\
1.64	-16.29\\
};
\addlegendentry{LQR min.}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
-1.64	8.91\\
-1.55	8.97\\
-1.45	8.95\\
-1.35	8.83\\
-1.26	8.63\\
-1.16	8.34\\
-1.06	7.97\\
-0.97	7.52\\
-0.87	7\\
-0.77	6.4\\
-0.68	5.75\\
-0.58	5.04\\
-0.48	4.27\\
-0.39	3.47\\
-0.29	2.63\\
-0.19	1.77\\
-0.1	0.89\\
0	0\\
0.1	-0.89\\
0.19	-1.77\\
0.29	-2.63\\
0.39	-3.47\\
0.48	-4.27\\
0.58	-5.04\\
0.68	-5.75\\
0.77	-6.4\\
0.87	-7\\
0.97	-7.52\\
1.06	-7.97\\
1.16	-8.34\\
1.26	-8.63\\
1.35	-8.83\\
1.45	-8.95\\
1.55	-8.97\\
1.64	-8.91\\
};
\addlegendentry{LQR max.}

\end{axis}

\begin{axis}[%
width=4.208in,
height=4.219in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> plots/pendulumv4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor2}{rgb}{0.00000,0.44706,0.74118}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.427in,
height=3.271in,
at={(0.583in,0.625in)},
scale only axis,
xmin=-3.14159265358979,
xmax=0,
xtick={-3.14159265358979,-2.3562,-1.5707963267949,-0.785398163397448,0},
xticklabels={{-3.14},{-2.36},{-1.57},{-0.79},{0}},
xlabel style={font=\color{white!15!black}},
xlabel={$\theta$},
ymin=-12,
ymax=21,
ylabel style={font=\color{white!15!black}},
ylabel={$u(\theta)$},
axis background/.style={fill=white},
title style={font=\bfseries},
title={$\text{(b) u(}\theta\text{) for different controllers}$},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
-3.19	2.38\\
-3.09	2.63\\
-3	2.88\\
-2.9	3.11\\
-2.8	3.32\\
-2.71	3.51\\
-2.61	3.67\\
-2.51	3.79\\
-2.42	3.87\\
-2.32	3.91\\
-2.22	3.89\\
-2.13	3.83\\
-2.03	3.7\\
-1.93	3.52\\
-1.84	3.27\\
-1.74	2.96\\
-1.64	2.59\\
-1.55	2.15\\
-1.45	1.65\\
-1.35	1.09\\
-1.26	0.46\\
-1.16	-0.21\\
-1.06	-0.94\\
-0.97	-1.72\\
-0.87	-2.54\\
-0.77	-3.39\\
-0.68	-4.27\\
-0.58	-5.18\\
-0.48	-6.1\\
-0.39	-7.03\\
-0.29	-7.95\\
-0.19	-8.87\\
-0.1	-9.77\\
0	-10.64\\
};
\addlegendentry{NL. optimal}

\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
-3.19	20.58\\
-3.09	19.62\\
-3	18.67\\
-2.9	17.71\\
-2.8	16.75\\
-2.71	15.79\\
-2.61	14.83\\
-2.51	13.88\\
-2.42	12.92\\
-2.32	11.96\\
-2.22	11\\
-2.13	10.04\\
-2.03	9.09\\
-1.93	8.13\\
-1.84	7.17\\
-1.74	6.21\\
-1.64	5.25\\
-1.55	4.3\\
-1.45	3.34\\
-1.35	2.38\\
-1.26	1.42\\
-1.16	0.46\\
-1.06	-0.49\\
-0.97	-1.45\\
-0.87	-2.41\\
-0.77	-3.37\\
-0.68	-4.33\\
-0.58	-5.28\\
-0.48	-6.24\\
-0.39	-7.2\\
-0.29	-8.16\\
-0.19	-9.12\\
-0.1	-10.07\\
0	-11.03\\
};
\addlegendentry{LQR min.}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
-3.19	3.63\\
-3.09	4.61\\
-3	5.5\\
-2.9	6.31\\
-2.8	7.02\\
-2.71	7.62\\
-2.61	8.12\\
-2.51	8.5\\
-2.42	8.77\\
-2.32	8.93\\
-2.22	8.96\\
-2.13	8.88\\
-2.03	8.67\\
-1.93	8.36\\
-1.84	7.93\\
-1.74	7.39\\
-1.64	6.76\\
-1.55	6.02\\
-1.45	5.2\\
-1.35	4.3\\
-1.26	3.33\\
-1.16	2.3\\
-1.06	1.21\\
-0.97	0.08\\
-0.87	-1.07\\
-0.77	-2.25\\
-0.68	-3.44\\
-0.58	-4.62\\
-0.48	-5.78\\
-0.39	-6.92\\
-0.29	-8.03\\
-0.19	-9.08\\
-0.1	-10.08\\
0	-11\\
};
\addlegendentry{LQR max.}

\end{axis}
\end{tikzpicture}%
